What are Attackers after on IoT Devices? An approach based on a multi-phased multi-faceted IoT honeypot ecosystem and data clustering

The growing number of Internet of Things (IoT) devices makes it imperative to be aware of the real-world threats they face in terms of cybersecurity. While honeypots have been historically used as decoy devices to help researchers/organizations gain a better understanding of the dynamic of threats on a network and their impact, IoT devices pose a unique challenge for this purpose due to the variety of devices and their physical connections. In this work, by observing real-world attackers' behavior in a low-interaction honeypot ecosystem, we (1) presented a new approach to creating a multi-phased, multi-faceted honeypot ecosystem, which gradually increases the sophistication of honeypots' interactions with adversaries, (2) designed and developed a low-interaction honeypot for cameras that allowed researchers to gain a deeper understanding of what attackers are targeting, and (3) devised an innovative data analytics method to identify the goals of adversaries. Our honeypots have been active for over three years. We were able to collect increasingly sophisticated attack data in each phase. Furthermore, our data analytics points to the fact that the vast majority of attack activities captured in the honeypots share significant similarity, and can be clustered and grouped to better understand the goals, patterns, and trends of IoT attacks in the wild.

==> section4.tex <==
\section{Multi-faceted and multi-phased deployment/experimentation}
\label{sec:multiphased}

%\hspace{\parindent}
For the purpose of this project, a multi-faceted approach was chosen.  Although, these honeypots provided satisfactory results, to have more specific information on IoT attacks, {\it HoneyCamera} designed and deployed along with others. Each one of these honeypots emulated at least one IoT device’s protocol, including {\it HTTP} and {\it SSH}, to name just two.
In addition, honeypots were deployed in different phases. The first phase had the least changes from the original software to start receiving attacks. From this point, honeypot ecosystem started to collect data, and the analyzed data helped to create the subsequent phase by understanding what cybercriminals are looking for, and how this ecosystem can become more sophisticated. The second phase was repeated many times until acceptable results were achieved. At the end, in phase three, previous information was used to create more advanced low interaction honeypots. In this section, these taken approaches are presented.

\begin{description}
\item[HoneyLogin] Cowrie honeypot was used to emulate a vulnerable IoT device with open SSH (port 22) or telnet (port 23). Three main honeypots' instances were created in three different phases, and Busybox OS was also picked for this purpose.
\begin{itemize}
  \item In the first phase, the system was allowed to accept every possible combination of usernames and passwords. Two honeypots were implemented, one in Singapore and the other one inside the university’s infrastructure.
  \item In the second phase which started after 6 months, the top 30 username/password combinations were picked with command execution to create a new honeypot instance inside the university's network. In addition, new usernames and file systems were created, and more bait was added to it. Accordingly, previous logs were analyzed, and all of the problems encountered in the first phase were fixed, such as \textit{file} command's response added to the honeypot configuration.
  \item In the last phase, all the information collected was used to create a more sophisticated honeypot. As a result, a complex password was generated, and the number of possible successful login combinations was limited to only one. Since the password was set to be very complicated, every successful login would imply that it was possibly done by a real hacker which consequently could provide valuable information.
\end{itemize}

\item[HoneyWindowsBox] Dionaea was the second installed honeypot for this purpose.
\begin{itemize}
\item In the first phase, a default version of Dionaea was installed through cloud infrastructure. Unfortunately, this version could not pass the vetting system and was easily found as a honeypot.
\item To achieve a hard detectable honeypot, in phase two, services were broken down into two different combinations. The first honeypot had FTP, HTTP and HTTPS services while only SMB and MSSQL services were enabled for the second one. Three locations were chosen to install Dionaea (India, Canada and the university's network). These IPs popped up as a real system in Shodan. KFSensor honeypot was the second honeypot that was installed during this step. For this purpose, an educational license was acquired from Keyfocus. Paris and the United States were chosen as the locations to install this honeypot.
\end{itemize}
\item[HoneyCamera] is the last implemented honeypot. Different cameras have different available ports.
\begin{itemize}
\item In the first phase, three honeypots were implemented. Two servers in Sydney and Paris had only port 8080 exposed while the other one in London had port 80. The first Two Honeypots were used to emulate D-Link DCS-5020L and the other one to imitate D-Link DCS-5030L camera.
\item In the second phase, a combination of HoneyCamera and HoneyLogin will be implemented. At this time, this process is still under development.
\end{itemize}
\end{description}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

